Infinite-Horizon Graph Filters: Leveraging Power Series to Enhance Sparse Information Aggregation

Graph Neural Networks (GNNs) have shown considerable effectiveness in a variety of graph learning tasks, particularly those based on the message-passing approach in recent years. However, their performance is often constrained by a limited receptive field, a challenge that becomes more acute in the presence of sparse graphs. In light of the power series, which possesses infinite expansion capabilities, we propose a novel Graph Power Filter Neural Network (GPFN) that enhances node classification by employing a power series graph filter to augment the receptive field. Concretely, our GPFN designs a new way to build a graph filter with an infinite receptive field based on the convergence power series, which can be analyzed in the spectral and spatial domains. Besides, we theoretically prove that our GPFN is a general framework that can integrate any power series and capture long-range dependencies. Finally, experimental results on three datasets demonstrate the superiority of our GPFN over state-of-the-art baselines.

==> 5_perfrom_ama.tex <==
% ama表
\begin{table*}[htbp]
  \centering
  \small
  \caption{Performance comparison on Amacomp and Amaphoto for node classification.
  %under different missing rates
  %Node classification performances of baselines on \textbf{Uniform \& Struct Missing} for Amacomp \& Amaphoto under different missing rates. 
  %The bold and underline marker denotes the best and second-best performance on each dataset.
  }
  \vspace*{-0.3cm}
  \begin{threeparttable}
    \resizebox{1.0\linewidth}{!}{\begin{tabular}{c|c|ccccc|ccccc}
    \hline
    \multirow{2}[3]{*}{Missing Type} & \multicolumn{1}{c|}{Dataset} & \multicolumn{5}{c|}{\textbf{AmaPhoto}} & \multicolumn{5}{c}{\textbf{AmaComp}} \\ 
\cline{2-12}          & \multicolumn{1}{c|}{Missing Rate} & 10\%   & 30\%   & 50\%   & 70\%   & 90\%   & 10\%   & 30\%   & 50\%   & 70\%   & 90\% \\ \hline
    \multicolumn{1}{c|}{\multirow{17}[2]{*}{\makecell[c]{ Uniform\\ Missing}}}
    &MF    & 91.83 & 91.50  & 90.77 & 89.47 & 79.83 & 83.97 & 83.60  & 82.67 & 81.23 & 62.41 \\
    &MFT*  & 92.23 & 91.88 & 91.15 & 88.28 & 75.73 & 82.82 & 82.05 & 80.76 & 77.11 & 49.42 \\
    &KNN*  & 92.27 & 91.94 & 91.37 & 90.03 & 81.91 & 82.89 & 82.18 & 81.54 & 79.34 & 66.04 \\
    &SOFTIMP* & 92.23 & 91.92 & 91.55 & 90.55 & 85.22 & 82.99 & 82.37 & 81.48 & 79.27 & 69.04 \\
    &VAE*  & 92.20  & 91.90  & 91.15 & 89.28 & 81.43 & 82.65 & 81.72 & 80.47 & 78.55 & 67.26 \\
    &GAE  & 89.77 &	87.87&	86.53& 84.25&	80.23 & 80.39&	78.73&	75.42&	72.20&	57.45\\
    &VGAE&  90.35&	89.22&	88.95	&86.04&	82.98& 81.82&	80.64&	77.69&	72.85&	62.85\\
    &GINN* & 92.25 & 91.87 & 91.14 & 88.59 & 79.80  & 82.94 & 82.27 & 80.89 & 76.46 & 58.34 \\
    &GAIN* & 92.23 & 91.90  & 91.15 & 89.28 & 81.43 & 82.94 & 82.44 & 81.56 & 79.96 & 76.15 \\
    &GCNMF & 92.39 & {92.24} & {91.79} & {91.01} & {89.80}  & \underline{86.13} & \underline{85.73} & \underline{85.47} & \underline{84.69} & \underline{80.47} \\
    &PaGNN & \underline{92.64} & 90.69 & 91.54 & 90.39 & \textbf{89.98} & 84.78 & 83.76 & 83.08 & 81.21 & 78.79 \\
    &SVGA & 91.69&	91.33&	89.49	&88.84	&84.77&  83.66&	83.11&	82.92&	81.44&	77.31 \\
    &GNN-AC &92.18	&91.53&	89.46	&87.44	&84.38 & 83.61	&81.58&	80.49	&78.39&	74.90\\ 
    &GCN-Katz & 88.50 & 	86.57	&85.92&	84.43&	79.36	&78.54	&75.11&	74.40&	71.37&	70.56\\
    &GAE-Katz & 90.79&	90.68&	88.86&	89.73&	78.15& 83.13&	85.04	&84.49&	83.24&	67.26\\
    \cline{2-12}          &{\M} & \textbf{92.96} & \textbf{92.73} & \underline{91.80} & \textbf{91.68} & 89.39 & \textbf{86.15} & \textbf{86.31} & \textbf{86.04} & \textbf{85.43} & \textbf{82.43} \\
    &{\M-Katz} & 92.41 & \underline{92.43} & \textbf{91.84} & \underline{91.25} & \underline{89.93} & {85.38} & {84.98} & {84.65} & {83.73} & {79.81} \\
    \hline
    \multicolumn{1}{c|}{\multirow{19}[2]{*}{\makecell[c]{ Structurally\\ Missing}}} & MF    & 91.77 & 91.07 & 90.03 & 88.87 & 81.53 & 84.17 & 83.50  & 82.27 & 79.01    & 51.40 \\
    &MFT*  & 92.08 & 91.59 & 90.56 & 87.58 & 77.69 & 82.48 & 81.43 & 79.40  & 75.19 & 27.33 \\
    &KNN*  & 92.04 & 91.43 & 90.37 & 88.80  & 80.48 & 82.59 & 81.57 & 80.25 & 76.91 & 42.23 \\
    &SOFTIMP* & 91.75 & 90.55 & 88.00    & 84.87 & 76.72 & 82.64 & 81.32 & 79.68 & 75.92 & 52.75 \\
    &VAE*  & 92.11 & 91.50  & 90.46 & 87.47 & 67.85 & 82.76 & 81.72 & 79.23 & 73.76 & 41.37 \\
    &GAE  & 90.57&	89.34&	88.20&	85.41&	77.87 & 81.54&	80.58&	77.60 &	74.11	&42.14 \\
    &VGAE  & 91.40&	90.08&	89.28	&87.47	&81.84  & 82.93	&80.73	&79.26&	73.52&	51.23 \\
    &GINN* & 92.09 & 91.53 & 90.43 & 87.77 & 77.14 & 82.55 & 81.46 & 79.59 & 75.08 & 26.10 \\
    &GAIN* & 92.04 & 91.49 & 90.63 & 88.60  & 76.48 & 82.76 & 82.11 & 80.76 & 74.38 & 54.20 \\
    &GCNMF & 92.21 & 91.00    & {90.87} & 89.69 & 86.09 & \underline{86.05} & \underline{85.78} & \underline{85.74} & \textbf{84.90} & {80.98} \\
    &PaGNN & {92.26} & {91.64} & 90.47 & \underline{90.21} & 86.59 & 84.84 & 84.54 & 84.19 & 82.64 & 79.92 \\
    &SAT  & 92.10  & 91.03 & 90.45 & 89.99 & {88.98} & 83.48 & 82.66 & 82.40  & 80.62 & 80.17 \\
    &ITR  &90.94&	90.01&	86.24	&85.60&	75.57&  83.52&	83.23	&82.33&	82.22&	80.14 \\
    &SVGA  &91.61	&91.11	&90.68	&87.51	&82.77 &83.84	&82.24	&81.25&	80.47&	79.84 \\
    &GNN-AC& 92.17	&91.25&	90.15&	88.22	&78.64 & 83.96&	81.15&	79.86	&78.30&	69.08 \\
    &GCN-Katz & 87.68&	86.07&	85.08	&84.78&	83.43& 80.25&	78.70&	75.98&	74.54&	73.93\\
    &GAE-Katz & 92.47&	84.72&	82.41	&86.52&	80.01 &81.84&	75.04&	75.11&	74.58&	72.03\\
\cline{2-12}          &{\M} & \textbf{92.55} & \textbf{92.15} & \textbf{92.14} & \textbf{90.69} & \underline{89.21} & \textbf{86.39} & \textbf{85.81} & \textbf{85.76} & \underline{84.39} & \textbf{82.18} \\
    &{\M-Katz} & \underline{92.46} & \underline{91.95} & \underline{91.23} & {89.49} & \textbf{89.80} & {85.03} &  85.31 & 84.92 & 83.21  & \underline{81.95} \\
    \hline
    \multicolumn{2}{c|}{Complete Attribute/ LP } & \multicolumn{5}{c|}{91.73/ 87.20}                 & \multicolumn{5}{c}{85.65/ 74.84} \\
    \hline
    %\multicolumn{2}{c|}{Label Propagation} & \multicolumn{5}{c|}{87.20}                 & \multicolumn{5}{c}{74.84} \\
    %\hline
    \end{tabular}}%
    % \begin{tablenotes}
    %   \footnotesize
    %     %  \item[1] ${}^\text{1}$Complete Attribute: 91.73, Label Propagation: 87.20 
    %     %  \item[2]  ${}^\text{2}$Complete Attribute: 85.65, Label Propagation: 74.84
    %     \item
    %     \qquad \qquad \qquad  \qquad \qquad \qquad \qquad \qquad \qquad 
    %      ${}^\text{1}$Complete Attribute: 91.73 \quad Label Propagation: 87.20\quad ${}^\text{2}$Complete Attribute: 85.65\quad Label Propagation:74.84
    %  \end{tablenotes}
    \begin{tablenotes}
    \footnotesize
    \item[*] The results are obtained from the previous work \cite{taguchi2021graph}.
    \end{tablenotes}
    \end{threeparttable}
  \label{tab:ama}%
  \vspace{-0.3cm}
\end{table*}%

% Ama-Uniform
% \begin{table*}[htbp]
% \caption{Performances of different approaches on \textbf{Uniform Missing} for Amacomp \and Amaphoto under different missing rates.}
% 	\label{tab:Amacomp_Amaphoto_uniform}
% 	\centering
% \begin{tabular}{c|ccccc|ccccc}

% \hline
% {  }                         & \multicolumn{5}{c|}{{  \textbf{Amacomp}${}^\text{1}$}}                                                                                                                                                                                                                     & \multicolumn{5}{c}{{  \textbf{Amaphoto}${}^\text{2}$}}                                                                                                                                                                                                                              \\ \cline{2-11} 
% \multirow{-2}{*}{{  Method}} & \multicolumn{1}{c|}{{  0.1}}            & \multicolumn{1}{c|}{{  0.3}}            & \multicolumn{1}{c|}{{  0.5}}                  & \multicolumn{1}{c|}{{  0.7}}            & {  0.9}            & \multicolumn{1}{c|}{{  0.1}}            & \multicolumn{1}{c|}{{  0.3}}            & \multicolumn{1}{c|}{{  0.5}}            & \multicolumn{1}{c|}{{  0.7}}            & {  0.9}            \\ \hline
% {  MF}                       & \multicolumn{1}{c|}{{  91.83}}          & \multicolumn{1}{c|}{{  91.5}}           & \multicolumn{1}{c|}{{  90.77}}                & \multicolumn{1}{c|}{{  89.47}}          & {  79.83}          & \multicolumn{1}{c|}{{  83.97}}          & \multicolumn{1}{c|}{{  83.6}}           & \multicolumn{1}{c|}{{  82.67}}          & \multicolumn{1}{c|}{{  81.23}}          & {  62.4}           \\
% {  VAE*}                     & \multicolumn{1}{c|}{{  92.2}}           & \multicolumn{1}{c|}{{  91.9}}           & \multicolumn{1}{c|}{{  91.15}}                & \multicolumn{1}{c|}{{  89.28}}          & {  81.43}          & \multicolumn{1}{c|}{{  82.65}}          & \multicolumn{1}{c|}{{  81.72}}          & \multicolumn{1}{c|}{{  80.47}}          & \multicolumn{1}{c|}{{  78.55}}          & {  67.26}          \\
% {  GAIN*}                    & \multicolumn{1}{c|}{{  92.23}}          & \multicolumn{1}{c|}{{  91.9}}           & \multicolumn{1}{c|}{{  91.15}}                & \multicolumn{1}{c|}{{  89.28}}          & {  81.43}          & \multicolumn{1}{c|}{{  82.94}}          & \multicolumn{1}{c|}{{  82.44}}          & \multicolumn{1}{c|}{{  81.56}}          & \multicolumn{1}{c|}{{  79.96}}          & {  76.15}          \\
% {  GCNMF}                    & \multicolumn{1}{c|}{{  \textbf{92.63}}} & \multicolumn{1}{c|}{{  {\underline {92.24}}}}    & \multicolumn{1}{c|}{{  {\underline {91.79}}}} & \multicolumn{1}{c|}{{  {\underline {91.01}}}}    & {  {\underline {89.8}}}     & \multicolumn{1}{c|}{{  {\underline {86.13}}}}    & \multicolumn{1}{c|}{{  {\underline {85.73}}}}    & \multicolumn{1}{c|}{{  {\underline {85.47}}}}    & \multicolumn{1}{c|}{{  {\underline {84.69}}}}    & {  {\underline {80.47}}}    \\
% {  PaGNN}                    & \multicolumn{1}{c|}{{  92.64}}          & \multicolumn{1}{c|}{{  90.69}}          & \multicolumn{1}{c|}{{  91.54}}                & \multicolumn{1}{c|}{{  90.39}}          & {  \textbf{89.98}} & \multicolumn{1}{c|}{{  84.78}}          & \multicolumn{1}{c|}{{  83.76}}          & \multicolumn{1}{c|}{{  83.08}}          & \multicolumn{1}{c|}{{  81.21}}          & {  78.79}          \\
% {  KNN*}                     & \multicolumn{1}{c|}{{  92.27}}          & \multicolumn{1}{c|}{{  91.94}}          & \multicolumn{1}{c|}{{  91.37}}                & \multicolumn{1}{c|}{{  90.03}}          & {  81.91}          & \multicolumn{1}{c|}{{  82.89}}          & \multicolumn{1}{c|}{{  82.18}}          & \multicolumn{1}{c|}{{  81.54}}          & \multicolumn{1}{c|}{{  79.34}}          & {  66.04}          \\
% {  MFT*}                     & \multicolumn{1}{c|}{{  92.23}}          & \multicolumn{1}{c|}{{  91.88}}          & \multicolumn{1}{c|}{{  91.15}}                & \multicolumn{1}{c|}{{  88.28}}          & {  75.73}          & \multicolumn{1}{c|}{{  82.82}}          & \multicolumn{1}{c|}{{  82.05}}          & \multicolumn{1}{c|}{{  80.76}}          & \multicolumn{1}{c|}{{  77.11}}          & {  49.42}          \\
% {  SOFTIMP*}                 & \multicolumn{1}{c|}{{  92.23}}          & \multicolumn{1}{c|}{{  91.92}}          & \multicolumn{1}{c|}{{  91.55}}                & \multicolumn{1}{c|}{{  90.55}}          & {  85.22}          & \multicolumn{1}{c|}{{  82.99}}          & \multicolumn{1}{c|}{{  82.37}}          & \multicolumn{1}{c|}{{  81.48}}          & \multicolumn{1}{c|}{{  79.27}}          & {  69.04}          \\
% {  GINN*}                    & \multicolumn{1}{c|}{{  92.25}}          & \multicolumn{1}{c|}{{  91.87}}          & \multicolumn{1}{c|}{{  91.14}}                & \multicolumn{1}{c|}{{  88.59}}          & {  79.8}           & \multicolumn{1}{c|}{{  82.94}}          & \multicolumn{1}{c|}{{  82.27}}          & \multicolumn{1}{c|}{{  80.89}}          & \multicolumn{1}{c|}{{  76.46}}          & {  58.34}          \\ \hline
% {  \M (ours)}               & \multicolumn{1}{c|}{{  {\underline {92.41}}}}    & \multicolumn{1}{c|}{{  \textbf{92.73}}} & \multicolumn{1}{c|}{{  \textbf{91.79}}}       & \multicolumn{1}{c|}{{  \textbf{91.68}}} & {  89.39}          & \multicolumn{1}{c|}{{  \textbf{86.15}}} & \multicolumn{1}{c|}{{  \textbf{86.31}}} & \multicolumn{1}{c|}{{  \textbf{86.04}}} & \multicolumn{1}{c|}{{  \textbf{85.43}}} & {  \textbf{82.43}} \\ \hline
% \end{tabular}

%     \begin{tablenotes}
%       \footnotesize
%         %  \item[1] ${}^\text{1}$Complete Attribute: 91.73, Label Propagation: 87.20 
%         %  \item[2]  ${}^\text{2}$Complete Attribute: 85.65, Label Propagation: 74.84
%         \item
%         \qquad \qquad \qquad  \qquad \qquad \qquad \qquad \qquad
%          ${}^\text{1}$Complete Attribute: 91.73, \quad    Label Propagation: 87.20;   \quad
%          ${}^\text{2}$Complete Attribute: 85.65, \quad Label Propagation: 74.84 
%      \end{tablenotes}

% \end{table*}

% C - Struct
% \begin{table*}[htbp]
% \caption{Performances of different approaches on \textbf{Struct Missing} for Cora \and Citeseer under different missing rates.}
% 	\label{tab:cora_citeseer_struct}
	
% \begin{tabular}{c|ccccc|ccccc}
% \hline
% {  }                         & \multicolumn{5}{c|}{{  \textbf{Cora}}}                                                                                                                                                                                                                                  & \multicolumn{5}{c}{{  \textbf{Citeseer}}}                                                                                                                                                                                                                          \\ \cline{2-11} 
% \multirow{-2}{*}{{  Method}} & \multicolumn{1}{c|}{{  0.1}}           & \multicolumn{1}{c|}{{  0.3}}           & \multicolumn{1}{c|}{{  0.5}}           & \multicolumn{1}{c|}{{  0.7}}           & {  0.9}                 & \multicolumn{1}{c|}{{  0.1}}            & \multicolumn{1}{c|}{{  0.3}}           & \multicolumn{1}{c|}{{  0.5}}           & \multicolumn{1}{c|}{{  0.7}}           & {  0.9}           \\ \hline
% {  MF}                       & \multicolumn{1}{c|}{{  80.96}}         & \multicolumn{1}{c|}{{  79.53}}         & \multicolumn{1}{c|}{{  76.67}}         & \multicolumn{1}{c|}{{  67.8}}          & {  35.13}               & \multicolumn{1}{c|}{{  70.27}}          & \multicolumn{1}{c|}{{  68.87}}         & \multicolumn{1}{c|}{{  63.23}}         & \multicolumn{1}{c|}{{  55.67}}         & {  27.3}          \\
% {  VAE*}                     & \multicolumn{1}{c|}{{  80.63}}         & \multicolumn{1}{c|}{{  78.57}}         & \multicolumn{1}{c|}{{  74.69}}         & \multicolumn{1}{c|}{{  60.71}}         & {  17.27}               & \multicolumn{1}{c|}{{  69.63}}          & \multicolumn{1}{c|}{{  66.34}}         & \multicolumn{1}{c|}{{  60.46}}         & \multicolumn{1}{c|}{{  40.71}}         & {  17.2}          \\
% {  GAIN*}                    & \multicolumn{1}{c|}{{  80.53}}         & \multicolumn{1}{c|}{{  78.36}}         & \multicolumn{1}{c|}{{  74.25}}         & \multicolumn{1}{c|}{{  61.33}}         & {  18.43}               & \multicolumn{1}{c|}{{  69.47}}          & \multicolumn{1}{c|}{{  65.88}}         & \multicolumn{1}{c|}{{  59.96}}         & \multicolumn{1}{c|}{{  41.21}}         & {  17.89}         \\
% {  GCNMF}                    & \multicolumn{1}{c|}{{  {\underline {81.65}}}}   & \multicolumn{1}{c|}{{  {\underline {80.67}}}}   & \multicolumn{1}{c|}{{  77.43}}         & \multicolumn{1}{c|}{{  {\underline {72.69}}}}   & {  {\underline {55.64}}}         & \multicolumn{1}{c|}{{  70.44}}          & \multicolumn{1}{c|}{{  66.57}}         & \multicolumn{1}{c|}{{  63.44}}         & \multicolumn{1}{c|}{{  56.88}}         & {  {{39.86}}}   \\
% {  PaGNN}                    & \multicolumn{1}{c|}{{  81.4}}          & \multicolumn{1}{c|}{{  80.52}}         & \multicolumn{1}{c|}{{  {\underline {77.46}}}}   & \multicolumn{1}{c|}{{  68.94}}         & {  54.75}               & \multicolumn{1}{c|}{{  {\underline {70.84}}}}    & \multicolumn{1}{c|}{{  68.84}}         & \multicolumn{1}{c|}{{  65.02}}         & \multicolumn{1}{c|}{{  56.86}}         & \underline {  {41.14}}         \\
% {  KNN*}                     & \multicolumn{1}{c|}{{  80.76}}         & \multicolumn{1}{c|}{{  78.63}}         & \multicolumn{1}{c|}{{  74.51}}         & \multicolumn{1}{c|}{{  63.29}}         & {  13.95}               & \multicolumn{1}{c|}{{  69.67}}          & \multicolumn{1}{c|}{{  66.09}}         & \multicolumn{1}{c|}{{  56.86}}         & \multicolumn{1}{c|}{{  19.51}}         & {  11.21}         \\
% {  MFT*}                     & \multicolumn{1}{c|}{{  80.91}}         & \multicolumn{1}{c|}{{  78.63}}         & \multicolumn{1}{c|}{{  74.47}}         & \multicolumn{1}{c|}{{  52.65}}         & {  17.05}               & \multicolumn{1}{c|}{{  69.84}}          & \multicolumn{1}{c|}{{  66.67}}         & \multicolumn{1}{c|}{{  51.08}}         & \multicolumn{1}{c|}{{  16.81}}         & {  15.75}         \\
% {  SOFTIMP*}                 & \multicolumn{1}{c|}{{  79.71}}         & \multicolumn{1}{c|}{{  69.31}}         & \multicolumn{1}{c|}{{  44.71}}         & \multicolumn{1}{c|}{{  36.68}}         & {  27.9}                & \multicolumn{1}{c|}{{  44.06}}          & \multicolumn{1}{c|}{{  25.83}}         & \multicolumn{1}{c|}{{  25.59}}         & \multicolumn{1}{c|}{{  25.41}}         & {  20.13}         \\
% {  GINN*}                    & \multicolumn{1}{c|}{{  80.85}}         & \multicolumn{1}{c|}{{  78.88}}         & \multicolumn{1}{c|}{{  74.76}}         & \multicolumn{1}{c|}{{  59.45}}         & {  13.92}               & \multicolumn{1}{c|}{{  69.64}}          & \multicolumn{1}{c|}{{  66.24}}         & \multicolumn{1}{c|}{{  55.76}}         & \multicolumn{1}{c|}{{  18.63}}         & {  12.32}         \\
% {  SAT*}                     & \multicolumn{1}{c|}{{  81.14}}         & \multicolumn{1}{c|}{{  80.11}}         & \multicolumn{1}{c|}{{  76.64}}         & \multicolumn{1}{c|}{{  71.48}}         & {  51.67}               & \multicolumn{1}{c|}{{  70.33}}          & \multicolumn{1}{c|}{{  {\underline {69.08}}}}   & \multicolumn{1}{c|}{{  {\underline {65.12}}}}   & \multicolumn{1}{c|}{{  {\underline {58.52}}}}   & {  34.32}         \\ \hline
% {  \M (ours)}               & \multicolumn{1}{c|}{{  \textbf{82.9}}} & \multicolumn{1}{c|}{{  \textbf{82.6}}} & \multicolumn{1}{c|}{{  \textbf{82.2}}} & \multicolumn{1}{c|}{{  \textbf{82.4}}} & {  \textbf{74.7(katz)}} & \multicolumn{1}{c|}{{  \textbf{71.56}}} & \multicolumn{1}{c|}{{  \textbf{70.6}}} & \multicolumn{1}{c|}{{  \textbf{69.8}}} & \multicolumn{1}{c|}{{  \textbf{66.5}}} & {  \textbf{58.5(katz)}} \\ \hline
% \end{tabular}
% \end{table*}

% Ama-Struct
% \begin{table*}[htbp]
% \caption{Performances of different approaches on \textbf{Struct Missing} for Amacomp \and Amaphoto under different missing rates.}
% 	\label{tab:Amacomp_Amaphoto_struct}
% 	\centering
% \begin{tabular}{c|ccccc|ccccc}
% \hline
% {  }                         & \multicolumn{5}{c|}{{  \textbf{Amacomp}}}                                                                                                                                                                                                                              & \multicolumn{5}{c}{{  \textbf{Amaphoto}}}                                                                                                                                                                                                                             \\ \cline{2-11} 
% \multirow{-2}{*}{{  Method}} & \multicolumn{1}{c|}{{  0.1}}            & \multicolumn{1}{c|}{{  0.3}}            & \multicolumn{1}{c|}{{  0.5}}            & \multicolumn{1}{c|}{{  0.7}}            & {  0.9}            & \multicolumn{1}{c|}{{  0.1}}            & \multicolumn{1}{c|}{{  0.3}}            & \multicolumn{1}{c|}{{  0.5}}            & \multicolumn{1}{c|}{{  0.7}}           & {  0.9}            \\ \hline
% {  MF}                       & \multicolumn{1}{c|}{{  91.77}}          & \multicolumn{1}{c|}{{  91.07}}          & \multicolumn{1}{c|}{{  90.03}}          & \multicolumn{1}{c|}{{  88.87}}          & {  81.53}          & \multicolumn{1}{c|}{{  84.17}}          & \multicolumn{1}{c|}{{  83.5}}           & \multicolumn{1}{c|}{{  82.27}}          & \multicolumn{1}{c|}{{  79}}            & {  51.4}           \\
% {  VAE*}                     & \multicolumn{1}{c|}{{  92.11}}          & \multicolumn{1}{c|}{{  91.5}}           & \multicolumn{1}{c|}{{  90.46}}          & \multicolumn{1}{c|}{{  87.47}}          & {  67.85}          & \multicolumn{1}{c|}{{  82.76}}          & \multicolumn{1}{c|}{{  81.72}}          & \multicolumn{1}{c|}{{  79.23}}          & \multicolumn{1}{c|}{{  73.76}}         & {  41.37}          \\
% {  GAIN*}                    & \multicolumn{1}{c|}{{  92.04}}          & \multicolumn{1}{c|}{{  91.49}}          & \multicolumn{1}{c|}{{  90.63}}          & \multicolumn{1}{c|}{{  88.6}}           & {  76.48}          & \multicolumn{1}{c|}{{  82.76}}          & \multicolumn{1}{c|}{{  82.11}}          & \multicolumn{1}{c|}{{  80.76}}          & \multicolumn{1}{c|}{{  74.38}}         & {  54.2}           \\
% {  GCNMF}                    & \multicolumn{1}{c|}{{  92.21}}          & \multicolumn{1}{c|}{{  91}}             & \multicolumn{1}{c|}{{  {\underline {90.87}}}}    & \multicolumn{1}{c|}{{  89.69}}          & {  86.09}          & \multicolumn{1}{c|}{{  {\underline {86.05}}}}    & \multicolumn{1}{c|}{{  {\underline {85.78}}}}    & \multicolumn{1}{c|}{{  {\underline {85.74}}}}    & \multicolumn{1}{c|}{{  \textbf{84.9}}} & {  {\underline {80.98}}}    \\
% {  PaGNN}                    & \multicolumn{1}{c|}{{  {\underline {92.26}}}}    & \multicolumn{1}{c|}{{  {\underline {91.64}}}}    & \multicolumn{1}{c|}{{  90.47}}          & \multicolumn{1}{c|}{{  {\underline {90.21}}}}    & {  86.59}          & \multicolumn{1}{c|}{{  84.84}}          & \multicolumn{1}{c|}{{  84.54}}          & \multicolumn{1}{c|}{{  84.19}}          & \multicolumn{1}{c|}{{  82.64}}         & {  79.92}          \\
% {  KNN*}                     & \multicolumn{1}{c|}{{  92.04}}          & \multicolumn{1}{c|}{{  91.43}}          & \multicolumn{1}{c|}{{  90.37}}          & \multicolumn{1}{c|}{{  88.8}}           & {  80.48}          & \multicolumn{1}{c|}{{  82.59}}          & \multicolumn{1}{c|}{{  81.57}}          & \multicolumn{1}{c|}{{  80.25}}          & \multicolumn{1}{c|}{{  76.91}}         & {  42.23}          \\
% {  MFT*}                     & \multicolumn{1}{c|}{{  92.08}}          & \multicolumn{1}{c|}{{  91.59}}          & \multicolumn{1}{c|}{{  90.56}}          & \multicolumn{1}{c|}{{  87.58}}          & {  77.69}          & \multicolumn{1}{c|}{{  82.48}}          & \multicolumn{1}{c|}{{  81.43}}          & \multicolumn{1}{c|}{{  79.4}}           & \multicolumn{1}{c|}{{  75.19}}         & {  27.33}          \\
% {  SOFTIMP*}                 & \multicolumn{1}{c|}{{  91.75}}          & \multicolumn{1}{c|}{{  90.55}}          & \multicolumn{1}{c|}{{  88}}             & \multicolumn{1}{c|}{{  84.87}}          & {  76.72}          & \multicolumn{1}{c|}{{  82.64}}          & \multicolumn{1}{c|}{{  81.32}}          & \multicolumn{1}{c|}{{  79.68}}          & \multicolumn{1}{c|}{{  75.92}}         & {  52.75}          \\
% {  GINN*}                    & \multicolumn{1}{c|}{{  92.09}}          & \multicolumn{1}{c|}{{  91.53}}          & \multicolumn{1}{c|}{{  90.43}}          & \multicolumn{1}{c|}{{  87.77}}          & {  77.14}          & \multicolumn{1}{c|}{{  82.55}}          & \multicolumn{1}{c|}{{  81.46}}          & \multicolumn{1}{c|}{{  79.59}}          & \multicolumn{1}{c|}{{  75.08}}         & {  26.1}           \\
% {  SAT*}                     & \multicolumn{1}{c|}{{  92.1}}           & \multicolumn{1}{c|}{{  91.03}}          & \multicolumn{1}{c|}{{  90.45}}          & \multicolumn{1}{c|}{{  89.99}}          & {  {\underline {88.98}}}    & \multicolumn{1}{c|}{{  83.48}}          & \multicolumn{1}{c|}{{  82.66}}          & \multicolumn{1}{c|}{{  82.4}}           & \multicolumn{1}{c|}{{  80.62}}         & {  80.17}          \\ \hline
% {  \M (ours)}               & \multicolumn{1}{c|}{{  \textbf{92.46}}} & \multicolumn{1}{c|}{{  \textbf{92.15}}} & \multicolumn{1}{c|}{{  \textbf{92.14}}} & \multicolumn{1}{c|}{{  \textbf{90.69}}} & {  \textbf{89.21}} & \multicolumn{1}{c|}{{  \textbf{86.39}}} & \multicolumn{1}{c|}{{  \textbf{85.81}}} & \multicolumn{1}{c|}{{  \textbf{85.76}}} & \multicolumn{1}{c|}{{  {\underline {84.39}}}}   & {  \textbf{82.18}} \\ \hline
% \end{tabular}
% \end{table*}


==> 7_rebuttal.tex <==
\section{Reviewer 1}
\section{Reviewer 3}
\section{Reviewer 4}
